Exclusion of Extreme Jurors and Minority Representation: The Effect of Jury Selection Procedures

We compare two jury selection procedures meant to safeguard against the inclusion of biased jurors that are perceived as causing minorities to be under-represented. The Strike and Replace procedure presents potential jurors one-by-one to the parties, while the Struck procedure presents all potential jurors before the parties exercise their challenges. Struck more effectively excludes extreme jurors but leads to a worse representation of minorities. The advantage of Struck in terms of excluding extremes is sizable in a wide range of cases. In contrast, Strike and Replace better represents minorities only if the minority and majority are polarized. Results are robust to assuming the parties statistically discriminate against jurors based on group identity.

==> graphics/tables.tex <==

Group-a represents 50\% of the jury pool 

Average fraction of minorities 	 & 	 0.48 	& 0.50 	& 0.49 	& 0.50 	& 0.50 	& 0.50 	& 0.50 \\
Standard deviation  		 & 	 0.18 	& 0.20 	& 0.16 	& 0.17 	& 0.15 	& 0.15 	& 0.14 \\
Fraction of juries with at least 1 	 & 	 0.99 	& 0.99 	& 1.00 	& 1.00 	& 1.00 	& 1.00 	& 1.00 \\

Group-a represents 25\% of the jury pool 

Average fraction of minorities 	 & 	 0.10 	& 0.07 	& 0.18 	& 0.16 	& 0.23 	& 0.23 	& 0.25 \\
Standard deviation  		 & 	 0.11 	& 0.11 	& 0.12 	& 0.12 	& 0.12 	& 0.12 	& 0.12 \\
Fraction of juries with at least 1 	 & 	 0.57 	& 0.45 	& 0.88 	& 0.84 	& 0.95 	& 0.95 	& 0.97 \\

Group-a represents 10\% of the jury pool 

Average fraction of minorities 	 & 	 0.02  	& 0.00 	& 0.05 	& 0.04 	& 0.09 	& 0.08 	& 0.10 \\
Standard deviation  		 & 	 0.04 	& 0.01 	& 0.07 	& 0.06 	& 0.08 	& 0.08 	& 0.09 \\
Fraction of juries with at least 1 	 & 	 0.17 	& 0.02 	& 0.47 	& 0.38 	& 0.66 	& 0.64 	& 0.71 \\
Representation in balanced groups  (table tab:betas-grouprep-balanced) 


\begin{tabular}{lccccccc}
	 Polarization &\multicolumn{2}{c}{Extreme}
 	 &\multicolumn{2}{c}{Moderate}
 	 &\multicolumn{2}{c}{Mild}
 	 & (All) \\
 	 Procedure    & \SAR & \STR  & \SAR & \STR  & \SAR & \STR  & \RAN \\
 	 \hline
     \multicolumn{8}{c}{$r=0.45$}
Average fraction of minorities 	 & 	 0.39 	& 0.40 	& 0.42 	& 0.42 	& 0.45 	& 0.44 	& 0.45 \\
Standard deviation  		 & 	 0.18 	& 0.20 	& 0.16 	& 0.17 	& 0.15 	& 0.15 	& 0.14 \\
\end{tabular}



\begin{tabular}{lccccccc}
	 Polarization &\multicolumn{2}{c}{Extreme}
 	 &\multicolumn{2}{c}{Moderate}
 	 &\multicolumn{2}{c}{Mild}
 	 & (All) \\
 	 Procedure    & \SAR & \STR  & \SAR & \STR  & \SAR & \STR  & \RAN \\
 	 \hline
     \multicolumn{8}{c}{Slightly asymmetric$
Average fraction of minorities 	 & 	 0.47 	& 0.50 	& 0.49 	& 0.49 	& 0.49 	& 0.49 	& 0.50 \\
Standard deviation  		 & 	 0.17 	& 0.20 	& 0.15 	& 0.16 	& 0.15 	& 0.16 	& 0.14 \\
\end{tabular}


 Appendix Table tab-app:betas-grouprep 

Average fraction of minorities 	 & 	 0.12 	& 0.08 	& 0.18 	& 0.16 	& 0.23 	& 0.23 	& 0.25 \\
Standard deviation  		 & 	 0.11 	& 0.11 	& 0.12 	& 0.12 	& 0.12 	& 0.12 	& 0.13 \\
Fraction of juries with at least 1 	 & 	 0.76 	& 0.45 	& 0.89 	& 0.84 	& 0.96 	& 0.95 	& 0.97 \\

Average fraction of minorities 	 & 	 0.01  	& 0.00 	& 0.05 	& 0.04 	& 0.09 	& 0.08 	& 0.10 \\
Standard deviation  		 & 	 0.03 	& 0.02 	& 0.06 	& 0.06 	& 0.08 	& 0.08 	& 0.09 \\
Fraction of juries with at least 1 	 & 	 0.09 	& 0.02 	& 0.44 	& 0.38 	& 0.66 	& 0.64 	& 0.72 \\
